HAMSTER: Hierarchical Action Models For Open-World Robot Manipulation

Large foundation models have shown strong open-world generalization to complex problems in vision and language, but similar levels of generalization have yet to be achieved in robotics. One fundamental challenge is the lack of robotic data, which are typically obtained through expensive on-robot operation. A promising remedy is to leverage cheaper, off-domain data such as action-free videos, hand-drawn sketches or simulation data. In this work, we posit that hierarchical vision-language-action (VLA) models can be more effective in utilizing off-domain data than standard monolithic VLA models that directly finetune vision-language models (VLMs) to predict actions. In particular, we study a class of hierarchical VLA models, where the high-level VLM is finetuned to produce a coarse 2D path indicating the desired robot end-effector trajectory given an RGB image and a task description. The intermediate 2D path prediction is then served as guidance to the low-level, 3D-aware control policy capable of precise manipulation. Doing so alleviates the high-level VLM from fine-grained action prediction, while reducing the low-level policy's burden on complex task-level reasoning. We show that, with the hierarchical design, the high-level VLM can transfer across significant domain gaps between the off-domain finetuning data and real-robot testing scenarios, including differences on embodiments, dynamics, visual appearances and task semantics, etc. In the real-robot experiments, we observe an average of 20% improvement in success rate across seven different axes of generalization over OpenVLA, representing a 50% relative gain. Visual results, code, and dataset are provided at: https://hamster-robot.github.io/

==> retired/intro_sim_story.tex <==
Large-scale imitation learning efforts have resulted in generalist policies able to perform manipulation tasks~\citep{robomimic2021,ravichandar2020recent}. However, these methods require lots of data, which is expensive and time-consuming to collect on real robots, and have difficulty generalizing to new tasks.
Our goal is to drastically reduce the data needed for real-world robotics while also enabling better generalization to new tasks.


One approach to reducing real-world data is training policies in simulation and transferring these policies to the real world. 
While this approach has worked well for navigation with restricted observation spaces [CITE RMA, Zurich paper, etc.], it's much more difficult to do so with visual manipulation policies as visual features trained in simulation don't transfer well to the real world, requiring very specific, hard-to-build simulators that reflect the exact real world scene [CITE STUFF]. Designing such sims for each new robot embodiment or environment setting is not scalable.
What if we could instead use arbitrary simulators that don't need to directly align with our downstream tasks and embodiment?
\caelan{This paragraph reads like the contribution is on the simulation side, not on the policy side}

To enable this, our key insight is to instead separate the policy into two levels, one that reasons about the task and one that actually performs low-level control. With this separation, the higher-level reasoner can be trained on general robotic simulation data to learn \emph{what} high-level actions to perform for various robot manipulation tasks. Meanwhile, the low-level control policy can instead learn \emph{how} to execute those high-level actions rather than focusing on specific visual features that do not generalize from sim to real.
\caelan{We'll need to cite a few hierarchical policy learning papers}

Specifically, we fine-tune Vision Language Models (VLMs)~\citep{bommasani2021opportunities}, pre-trained on large amounts of visual data, on general robotic simulation data to learn \emph{what} high-level actions are useful in robot manipulation. In contrast with works that directly fine-tune VLMs for low-level actions [RT-2~\citep{brohan2022rt,zitkovich2023rt}, OpenVLA~\citep{kim2024openvla}, LLARVA~\citep{niu2024llarva}]---which still require far too much data to perform well---we fine-tune VLMs to output easy-to-generalize, high-level trajectory sketches that can be fed to any downstream visual policy. These sketch-level representations have been shown to enable better task generalization while requiring less robot-specific data~\citep{gu2023rttrajectory}.

Our key contribution is a pipeline that can be trained on \emph{general} robotic simulation data, then with very small amounts of downstream real-robot data, guides any visual policy to simply focus on the low-level actions needed for control.
\caelan{If the focus is is on the hybrid simulation and real training, the most critical thing to do is obtain some real-world results that back up that it works}

\textbf{Our contributions are as follows:}
\begin{itemize}
    \item A novel hierarchical policy architecture that uses a VLMs to make high-level decisions and, conditioned on these decisions, deploys RVT for low-level control.
    \item A data efficient training regime that leverages simulation data to train the high level and real data to train the low level.
    \item Simulation and real experiments ...
\end{itemize}

==> sections/experiments_workshop.tex <==
\section{Experimental Evaluation}


To test the hypotheses proposed in Section~\ref{sec:method}, we perform empirical evaluations in both simulation and the real world. %The experiments primarily aim to answer the following questions: (1) do hierarchical VLA models enable behavioral generalization to unseen scenarios? (2) do hierarchical VLA models show more effective cross-domain generalization than monolithic VLA models or low-level imitation learning methods? (3) is behavior learned by hierarchical VLA models robust to significant degrees of visual and semantic variations? (4) does including cross-domain data from settings like simulation really help with model generalization? (5) does explicitly finetuning the high-level VLM yield benefits in terms of spatial and semantic reasoning?

%\ankit{shall we remove this paragraph}
%To validate these hypotheses, we perform experiments in simulation by training both the high-level VLM and the low-level 3D policy on data from the RLBench~\citep{james2020rlbench} benchmark environment and testing on visual and semantic variations in the related Colloseum benchmark~\cite{pumacay2024colosseum}. In the real world, we perform experiments by training the base VLM model, VILA-1.5-13b~\citep{vila2024}, on the data mixture proposed in Section~\ref{sec:method:vlm:datasets}, and testing on a completely unseen tabletop manipulation setting that is depicted in Fig [TODO]. Further details of the experimental setup in both simulation and the real world is provided in the following sections. 
%\ag{We need to have a figure of the table top setting clearly indicated}

\subsection{Real World Evaluation on Tabletop Manipulation}
\input{tables/real}
Our real-world evaluation experiments aim to test the generalization capability of hierarchical VLA models across significant semantic and visual variations. In particular, we consider a variant of \method\ that uses a VLM (VILA-1.5-13b) finetuned on the data mixture in Section~\ref{sec:method:vlm:datasets} as the high-level predictor, with a 3-D policy architecture - RVT-2~\citep{goyal2024rvt} as the choice of low-level policy, as described in Section~\ref{sec:method:policy}. The low-level 3D policy is trained with 320 episodes collected via teleoperation directly on the table-top manipulation setup shown in Fig.~\ref{fig:experiments:training_data}. Importantly, the high-level VLM in \method\ is not finetuned on any in-domain data and is directly transferred only from the cheap data sources described in Section~\ref{sec:method:vlm:datasets}. This suggests that any generalization that the VLM sees does not result from in-domain training data rather than from cross-domain transfer. 

% \ag{Ensure we have something showing the difference between training domains and testing setup. This is important to show the tranfer results.}

\textbf{Baseline comparisons.} We compare \method\ to a state-of-the-art monolithic VLA, OpenVLA~\citep{kim2024openvla}, as well as a non-VLM 3D imitation learning policy. For fair comparison, we finetune OpenVLA on the collected in-domain trajectory data described above since OpenVLA showed poor zero-shot generalization. For the 3D imitation learning policy, we use RVT-2~\citep{goyal2024rvt} as our baseline, as it is effective in learning robust policies with few demonstrations. The RVT-2 baseline is trained with the same teleoperation data used to train the low-level policy in \method\ but without the intermediate 2D path representation from \method 's VLM.

\begin{figure}[!tb]
    \centering
    %\includegraphics[width=\linewidth,trim={0in 4.8in 0in 0.5in},clip]{figs/main_exp_fig_short.pdf}
    \includegraphics[width=\linewidth]{figs/main_exp_fig_short.pdf}
    % \includegraphics[width=\linewidth,trim={1in 1.5in 3in 0.8in},clip]{figs/main_exp_fig.pdf}
    \caption{\footnotesize{Quantitative evaluation results on a real-world robot, evaluated across different axes of generalization. Across all generalization axes, \method \ outperforms monolithic VLAs and 3D imitation learning.}}
    \label{fig:experiments:main_exp}
    \vspace{-4mm}
\end{figure}

\textbf{Results.} Figure~\ref{fig:experiments:main_exp} summarizes our real-world results. We compile results for multiple task types, including `pick and place,' and nonprehensile tasks such as `push buttons' and `knock down objects.' Similar to prior work~\citep{kim2024openvla}, we test generalization across various axes: \emph{arrangement}: new positions and object combinations with seen objects; \emph{obj and goal:} unseen object-goal combinations; \emph{visual:} visual changes in table texture, lighting, distractor objects; \emph{language:} unseen language instructions (e.g., candy $\rightarrow$ sweet object); \emph{spatial:} unseen spatial object relationships in the instruction; \emph{novel object:} unseen objects; and lastly, \emph{multiple:} a combination of multiple variations. 
In total, we evaluate each model on 74 tasks for 222 total evaluations.
% \ag{It'd be really useful to have a figure demonstrating each of these variations}

We find that \method~is able to outperform monolithic VLA models as well as 3D imitation learning methods. This is significant because this improved performance is in the face of considerable visual and semantic changes in the test setting, showing the ability of \method~to transfer much more effectively than monolithic VLA models or non-VLM base models. See \Cref{sec:appendix:real_world_exp_details} for evaluation conditions, a task list, and other experiment details, and \Cref{sec:appendix:failure_modes} for failure modes.
Finally, see \Cref{sec:appendix:simulation_results} for results in simulation.
%We refer readers to the supplementary website for additional details on the failure modes and evaluation conditions. \jz{TODO: replace this with link to appendix section}

\subsection{Impact of Design Decisions on VLM performance}
\label{sec:experiments:vlm_design}
To better understand the transfer and generalization performance of the proposed hierarchical VLA model, we analyze the impact of various decisions involved in training the high-level VLM. We conduct a human evaluation of different variants of a trained high-level VLM on a randomly collected dataset of real-world test images, as shown in \Cref{fig:vlm_generalization}. We ask each model to generate 2D path traces corresponding to instructions such as ``move the block on the right to Taylor Swift'' 
%or ``screw the light bulb in the lamp'' 
(the full set is in \Cref{sec:appendix:generalization}). We then provide the paths generated by each method to human evaluators who have not previously seen any of the models' predictions. The human evaluators then rank the predictions for each method; we report the average rank across the samples in \Cref{tab:experiments:vlm}. 

We evaluate the following VLM models: (1) zero-shot state-of-the-art closed-source models such as GPT-4o using a similar prompt to ours (shown in \Cref{fig:gpt4o-prompt}), (2) zero-shot state-of-the-art closed-source models such as GPT-4o but using Code-as-Policies~\citep{liang2023code} to generate paths as described in \citet{gu2023rttrajectory} (prompt in \Cref{fig:cap-prompt}),
%(3) zero-shot open-source models (VILA-1.5-13b), without any finetuning, 
(3) finetuned open-source models (VILA-1.5-13b) on the data sources described in Section~\ref{sec:method:vlm:datasets}, but excluding the simulation trajectories from the RLBench dataset, (4) finetuned open-source models (VILA-1.5-13b) on the data sources described in Section~\ref{sec:method:vlm:datasets}, including path sketches from the RLBench dataset. The purpose of these evaluations is to first compare with closely related work that generates 2D trajectories using pretrained closed source VLMs~\cite{gu2023rttrajectory} (Comparison (1) and (2)). 
%Secondly, the comparison with (3) is meant to analyze the impact of finetuning over using zero-shot open-source VLMs for path generation. 
The comparison between (3) and (4) (our complete method) is meant to isolate the impact of including the simulation path sketches from the RLBench dataset. In doing so, we analyze the ability of the VLM to predict intermediate paths to transfer across significantly varying domains (from RLBench to the real world). 

The results suggest that: (1) zero-shot path generation, even from closed-source VLMs~\cite{gu2023rttrajectory} such as GPT-4o with additional help through Code-as-Policies~\citep{liang2023code}, underperforms VLMs finetuned on cross-domain data as in \method; (2) inclusion of significantly different training data such as low-fidelity simulators during finetuning improves the real-world VLM performance. This highlights the transferability displayed by \method\ across widely varying domains. These results emphasize that despite considerable perceptual differences, the \method's hierarchical VLA can effectively utilize diverse sources of cheap prior data for path predictions. 


\input{tables/vlm_workshop}


% We first study how fine-tuning \method s VLM on our curated datasets affects its performance. We find the fine-tuning the VLM on our curated robotic dataset significantly improves performance as shown in Table.~\ref{tab:vlm}.

% We also compare \method s fine-tuned VLM to techniques used in prior works for generating intermediate representations like 2D paths. Specifically, we compare to techniques used in RT-Trajectory: zero-shot VLM prompting and Code-as-policies. To accommodate the best-case scenario in prior works, we allow them to use state-of-the-art closed-source VLM, while our method is limited to open-source methods that can be finetunes. As illustrated in Table~\ref{tab:real}, we find that...

% Further, we examine the cross-domain generalization of \method s VLM. This is done by training on the RLBench simulation, which looks very different from the real world. We then test in the real world on tasks with semantics similar to tasks present in RLBench. Surprisingly, we find that \method is able to understand the underlying semantics of tasks from data is visually very different. This paves a path of effectively utilizing diverse sources of data.

%\paragraph{Significantly Out-of-Domain Scenarios}
%We further probe the VLM to study its generalization on setups that are ``significantly" out-of-domain. Figure~\ref{fig:vlm_generalization} shows some samples. Overall, we find the finetuned VLM in \method~ to be surprisingly robust on data that is significantly out-of-domain. For example, the finetuned VLM can draw reasonable 2D paths on hand-drawn sketches which were neither in the pre-training nor the finetuning data. We also ask the VLM to create 2D paths in cases that require world knowledge, like ``move the left block on Jensen Huang's photo". This is interesting as it shows that \method s VLM can utilize its knowledge from different domains (like knowledge about people). 

% \ag{I don't quite get this celebrity thing, can someone clarify this?}


% \ag{Overall we need to go through the experiments and really illustrate how different training and test are, illustrate the different testing conditions, illustrate some paths drawn by the VLM, and for the human comparison provide one illustrative example.}

==> sections/intro_ag.tex <==
\section{Introduction}
% VLM based learning methods
\begingroup
\renewcommand{\thefootnote}{}
\endgroup
Developing general robot manipulation policies has been notoriously difficult. With the advent of large vision-language models (VLMs) that display compelling examples of generalization, there is optimism that similar techniques can be helpful for robotic manipulation. A line of prior work~\citep{team2024octo, kim2024openvla, gu2023rttrajectory} builds open-world vision-language-action models (VLAs) by finetuning off-the-shelf, pretrained VLMs. \anqi{does rt-trajectory really fall under this category?} The recipe for training many of these VLA models has been to collect and curate a large-scale robotics-specific dataset, complete with images and corresponding on-robot actions\anqi{what about proprio}, and then finetune a VLM to directly produce actions~\citep{kim2024openvla,rt22023arxiv}. Such VLAs have shown robustness on simple tasks and controlled environmental variations. However, these models display limited generalization in terms of environment, object, task, and semantic variation. This issue could be attributed to the relative scarcity of diverse, in-domain training data\anqi{seems conflicting with previous sentence, claiming that they've already curated `large-scale' datasets}. The data needed to train these models is expensive since it requires end-to-end image-action pairs \anqi{isn't it the same for imitation learning models?} that must all be collected directly on-robot through an expensive medium such as teleoperation. A solution for training VLA models must be developed to instead learn from easy-to-collect ``cheap" sources of data. \anqi{should probably mention about 3D as well}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/robolines_teaser.pdf}
    \caption{\footnotesize{Overview of \method, VLAs and ``smaller" imitation learning methods. \method 's hierarchical design results in better generalization with a small amount of in-domain data. \method\ is able to utilize cheap training sources such as videos or simulations for enhanced generalization.}}
    \label{fig:teaser}
\vspace{-8mm}
\end{figure*}

% Imitation learning methods and their flaws
On the other hand, relatively ``small" \anqi{excessive use of quotation marks?} imitation learning models have shown impressive dexterity and geometric robustness. Such models have demonstrated promise across a range of complex tasks involving contact-rich manipulation and 3D reasoning, spanning domains from tabletop manipulation~\citep{shridhar2023perceiver,goyal2023rvt} to fine dexterous manipulation~\citep{zhao23aloha}\anqi{is aloha appropriate here? maybe?}. Trained on relatively small datasets, these models show local robustness and stable control \anqi{stable is vague} but typically lack semantic or visual generalization. They are often brittle to changes in the environment, semantic description of the tasks, or changes in the objects being manipulated~\citep{pumacay2024colosseum}. Reliable, generalizable robotic learning techniques must marry the generalization benefits of large VLMs, with the efficiency, local robustness and dexterity of small imitation learning policies, all while being able to train from abundant and cheap sources of data\anqi{seems over-claiming as the low-level policy is not trained with these cheap data}. In this work, we ask -- can we design VLA models that train on relatively abundant and cheap data sources\anqi{again, over-claiming}, showing broad visual and semantic generalization, while retaining the low-level geometric and 3D understanding displayed by small imitation learning models? \anqi{3D is not neccesarily guaranteed in ALOHA is an instance of a small model}

We propose that a hierarchical architecture for vision language action models, \method (\methodlong), can serve as an effective way to learn from abundant and inexpensive off-domain sources of data such as videos or simulation\anqi{Again, could be confusing with data source}. We study a family of \method s, where finetuned VLMs are connected to low-level 3D policy learning methods \anqi{3D policy seems to come out of nowhere} via intermediate 2D path representations. Since these 2D paths can easily be obtained in abundance from data sources such as videos or simulations (either with point tracking, hand-sketching, or proprioceptive projection)\anqi{cite}, these can be used to finetune the larger \anqi{? than what} higher-level VLM in \method. These 2D paths can then serve as guidance for a low-level policy that operates on rich 3D and proprioceptive inputs, alleviating the burden of long-horizon planning and semantic reasoning\anqi{this is important but not mentioned in the previous paragraph}, allowing low-level policies to focus on robustly generating precise, spatially-aware actions. 

Representations similar to 2D paths has been explored in the robot learning literature~\citep{gu2023rttrajectory}, primarily as a technique for flexible task specification. However, the key hypothesis explored in this paper is distinct -- we posit that using cheap data such as videos or simulation to finetune \emph{hierarchical} path generating VLMs can enable a surprising degree of cross-domain transfer \anqi{fact check this} as compared to the direct transfer of monolithic vision-language-action models ~\citep{brohan2022rt, kim2024openvla}. Here the focus is less on using paths as a scalable \anqi{?} technique for task specification, and more on using hierarchy as a mechanism for robust cross-domain transfer across settings with considerable visual and semantic differences. Specifically, we find that VLMs trained to predict 2D path representation can transfer to the real world from simulations that look very different from the real world\anqi{confusing sentence}, or across real-world scenarios with widely varying appearance\anqi{mention hand tracking?}. Hence, the hierarchical design of \method\ provides a way to utilize cheaper, but perceptually varying sources of ``off-domain'' data (such as simulation or cross-embodiment data) to benefit real-world control policies. 

% Ankit: Another option, although not very crisp and clear
The hierarchical design presented in \method\ can also offer additional advantages through the decoupling of VLM training and low-level action prediction. Specifically, since the higher-level VLM is predicting semantically meaningful trajectories from monocular RGB camera inputs, the lower-level control policies can operate from rich 3D and proprioceptive inputs. In doing so, \method\ inherits the semantic reasoning benefits of VLMs along with the 3D reasoning and spatial awareness benefits of 3D imitation learning policies ~\citep{goyal2024rvt, ke20243d}. Finally, since \method\ is built on both open-source VLMs and low-level policies, it can serve as a fully open-sourced enabler for the community-building vision-language-action models. \anqi{need merge with previous paragraph}

\anqi{mention viable action frequency of HAMSTER and monolithic VLA model, resp.}

==> sections/intro_ankit_yi.tex <==
\section{Introduction}


%%%%%% Hierarchical Action Model Story

\ankit{Large action models are looking promising for open world manipulation -- Talk about RTs, Octo, OpenVLA -- what large action models promise}

\ankit{Limitations in building large action models -- requires lots of data -- sim2real hasn't worked with them either -- they are also not very precise as compared to smaller skill specific models like RVT-2 -- huge compute requirements, latency issues}

\ankit{However, we have able to utilize internet scale data to create VLMs -- therefore can be we do something that allows us to use all this advancement to deliver open-world manipulation capabilities}

\ankit{Our proposal -- A hierarchical design that allows for much flexibility -- communication via an informed trajectory -- decouples the perception + semantic understanding from low level actions }

\ankit{We study an instantiation of this idea and show -- results -- highlight how we can use low-cost data / sim data -- highlight latency advantages}

\ankit{Contrast our work with others including RT-Trajectory}

\ankit{Summarize Contributions - General Hierarchical Design -- Explore the advantages and design choices for this design - Do experiments comparing stuff}

%%%%%% Cheap Data Story

\yi{I think maybe we can focus the story on cheap data and expensive data? A draft as below.}

Title \#1: Divide and Conquer: A Two-Part Framework for Data-Efficient and Generalizable Robotic Learning

\yi{maybe RoboDC: Data-Efficient and Generalizable Robotic Learning in a Divide and Conquer way}

Title \#2: Maximizing Generalization with Minimal Teleoperation Data: A Dual-Module Approach

Title \#3: Leveraging Inexpensive Data for Precision and Generalization in Robotic Skill Acquisition

Recent advances in robotic learning have seen VLA frameworks (cite RT-1, RT-2, RT-X, OpenVLA) achieve remarkable success, demonstrating strong generalization capabilities. However, a significant limitation of these VLA-style models are their reliance on large amounts of teleoperation data—typically hundreds of demonstrations—to learn new skills. 
\caelan{Express in terms of reported human hours and/or monetary cost, e.g. Google collected 18 months of data with a large team of human contractors for RT-1}
Despite various efforts to streamline this data collection process (cite ALOHA, AR2D2, UMI), these methods often still require access to real-world environments, special requirements and even the involvement of professional operators, which restricts the scalability of data collection compared to fields like computer vision or natural language processing, where tasks can be easily outsourced to large-scale annotators.

In contrast, behavior cloning methods such as RVT and 3DDA have shown that new skills can be learned with much smaller datasets—on the order of tens of demonstrations. \caelan{``In contrast'' - RT-1 is a BC approach} \caelan{RVT as published isn't really a high-frequency BC approach (waypoints)}
\yi{maybe we can also talk about some RL method which can learn do sim2real?} However, these approaches suffer from poor generalization and a lack of semantic understanding, limiting their ability to handle diverse or unseen tasks.
\caelan{Low task diversity in practice}

In this paper, we propose a novel framework that addresses the shortcomings of both approaches by dividing the problem into two parts. The first part, a high-level module, leverages large amounts of inexpensive data and is responsible for perception, language understanding, and planning. 
The second part, a shallow execution head, uses a limited amount of expensive data to perform accurate and robust actions based on high-level instructions. This combination allows our system to achieve strong generalization with minimal expensive data, similar to OpenVLA, while retaining the precision and robustness of behavior cloning methods.
\caelan{Define inexpensive and expensive}

\textbf{The main contributions of this paper are as follows:}
\begin{itemize}
    \item We propose a framework that strategically separates data into inexpensive and expensive sources, demonstrating that this approach reduces the need for costly teleoperation data while maintaining competitive performance.
    \item We show that our framework achieves the strong generalization ability of OpenVLA while retaining the accuracy and robustness of behavior cloning methods.
    \item We demonstrate that our method can also benefit from simulated data—another source of inexpensive data—by successfully transferring skills learned in simulation to real-world tasks.
\end{itemize}

\caelan{Needs more specifies (e.g. the trajectory prediction process)}

==> sections/method_workshop.tex <==
\section{\method: Hierarchical Action Models for Robotic Learning}
\label{sec:method}

In this work, we examine how VLA models can be trained on relatively abundant data to demonstrate cross-domain transfer capabilities, as opposed to training on expensive image-action data collected on a robot. \method\ is a family of hierarchical action models designed for this purpose, exhibiting generalizable and robust manipulation. It consists of two interconnected models: first, a higher-level VLM that is fine-tuned on large-scale, cross-modal data to produce intermediate guidance (detailed in \Cref{sec:method:vlm}), and second, a low-level policy that produces actions conditioned on the VLM's predicted guidance (detailed in \Cref{sec:method:policy}). The finetuned VLM and the low-level policy communicate using a 2D path representation. \Cref{fig:method} provides an overview of \method's design. Crucially, we study the ability of such a hierarchical design to enable training on cheap, abundantly available data such as simulation and videos. 

\textbf{Background: Imitation Learning via Supervised Learning.} The goal of imitation learning is to train a probabilistic policy $\pi_\theta(a \mid s, o, z)$ from an expert-provided dataset. This policy $\pi_\theta$ outputs the probability of producing action $a$ conditioned on proprioceptive states $s$, perceptual observations $o$, and language instructions $z$ that specify the task. In the typical imitation learning setting, a dataset of expert in-domain trajectories is provided, consisting of observation-action-language tuples $\mathcal{D} = \{(s_i, a_i, o_i, z_i)\}_{i=1}^N$. This dataset can be utilized to learn the parameters of the policy $\pi_\theta$. While $\pi$ can take on a variety of architectures with various training objectives~\citep{goyal2023rvt, ke20243d, zhao23aloha, chi23diffusion}, most imitation learning algorithms are trained via supervised learning to maximize the objective: $\mathbb{E}_{(s_i, a_i, o_i, z_i) \sim \mathcal{D}} \left[ \log \pi_\theta\left(a_i \mid s_i, o_i, z_i \right) \right].$ This core objective can be modified with rich architectural choices such as 3D policy architectures~\citep{goyal2023rvt, ke20243d} or more expressive policy distribution classes~\citep{zhao23aloha, chi23diffusion}, but generalization to out-of-domain to settings with semantic or visual variations is still challenging. We study how vision-language models can be used to aid the generalization of such low-level imitation learning-based policies.

\textbf{Problem Definition.}
Rather than operating in the pure imitation learning setting as described earlier, we study a scenario where cross-domain data is utilized to train VLA models. While the typical imitation learning setting uses a dataset of optimal in-domain, on-robot tuples $\mathcal{D} = \{(s_t, a_t, o_t, z_t)\}_{t=1}^N$ to learn a near-optimal policy $\pi_\theta$, in this setting we additionally assume access to a much larger dataset(s) of ``off-domain" approximately optimal data $\vlmdata = \{(o_i^o, z_i^o)\}_{i=1}^M$, where $M \gg N$, such as video or simulation data. This ``off-domain" data $\vlmdata$ is different from in-domain data $\mathcal{D}$ in several important ways: \emph{1)} Off-domain perceptual observations $o_i^o$ may be considerably different than in-domain perceptual observations $o_i$, even when the underlying physical state of the system is similar
% \footnote{Viewed from the lens of a partially observable Markov decision process, this involves differing emission functions across domains.}.
An illustrative example of this is the marked difference between simulation and real-world scene appearance (see Figure.~\ref{fig:vlm_generalization}). \emph{2)} The underlying physical dynamics of the system can be potentially different, i.e the transition dynamics $\mathds{P}(s'|s, a)$ between states $s', s$ may be different between off-domain sources such as video or simulation than the test-time deployment setting. While the dynamics may show level differences, we assume the higher-level coarse strategies to solve the task remain invariant. \emph{3)} Off-domain data may not have access directly to actions $a$ or proprioception $p$, for instance in video based datasets. This poses challenges to directly applying the standard imitation learning paradigm for these datasets.
% \anqi{Do we want to talk about different modalities, e.g., 2d single images versus 3d point clouds at all here?}

The goal is to leverage the combination of a small amount of ``expensive" in-domain data $\mathcal{D}$ and a large amount of relatively ``cheap" off-domain data $\vlmdata$ to obtain a generalizable policy $\pi_\theta$ that can be successfully deployed over various initial conditions, task variations, and visual variations in the in-domain robot environment. Without additional assumptions, this problem is arduous due to the lack of alignment between the in-domain and off-domain settings. In this work, we assume access to an intermediate \emph{path-labeler} $p_i = h(o_i, z_i)$ at training time, that accepts an observation $o_i$ and a language instruction $z_i$ from either the off-domain or in-domain datasets, to produce an intermediate path label $p_i$ that indicates \emph{how} to optimally perform the task $z_i$ from the observation $o_i$. In this work, we choose this intermediate path label $p_i$ to be a sequence of points, a 2D path, on the image that indicates coarse end-effector motion to solve the designated task. 
% \anqi{Should mention that it additionally include gripper actions. And ideally refer to a figure.} 
This path-labeler at training time can come from different sources --  a projection of known proprioception if available, human-drawn trajectory annotations on images, point-tracked end-effector or hand positions from video, and so on. Applying such a path labeler to the off-domain dataset yields $\Tilde{\vlmdata} = \{(o_i^o, z_i^o, p_i^o)\}_{i=1}^M$.
% while applying it to the in-domain dataset correspondingly yields $\Tilde{\mathcal{D}} = \{(s_i, a_i, o_i, z_i, p_i)\}_{i=1}^N$.
% \anqi{a small detail, for in-domain dataset, shouldn't eef projection be sufficient?}
% \jz{the path labeler $h$ notation is incorrect and doesn't align with the method description. notation here needs to change and be incorporated in \Cref{sec:method:policy:training}}\anqi{Ideally, we may actually want to use a different notation for datasets with path labels and without, e.g., $\mathcal{D}_\text{off}$ and $\Tilde{\mathcal{D}}_\text{off}$.}

% In the following sections, we propose and discuss a family of VLA architectures that finetune high-level VLMs to produce the above mentioned path labels $p_i$ from off-domain data $\Tilde{\vlmdata}$, that can then provide guidance to low-level policies trained from in-domain data $\mathcal{D}$. Importantly, we show that these types of architectures enjoy the ability to train on more easily available data sources such as video or simulation and demonstrate significant cross-domain generalization. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/robolines_method.pdf}
    \caption{\footnotesize{Depiction of \method 's execution. The high-level VLM is called once to generate the 2D path. The low-level policy is conditioned on the 2D path and interacts with the environment sequentially to execute low-level actions. The path predicted by the VLM enhances the low-level policy generalization capability.}
    }
    \vspace{-4mm}
    \label{fig:method}
\end{figure*}

\subsection{\method 's VLM for producing 2D Paths Trained from Off-Domain Data}
\label{sec:method:vlm}

The first stage of building a \method\ VLA model is finetuning a high-level VLM that predicts coarse 2D paths $p$ given a language instruction $z$ and observation $o$. This path represents the approximate trajectory of the robot end-effector on the input camera image. It also contains information about the gripper state (where to open the gripper and where to close it) as subsequently explained.

Although, conceptually, any VLM can be used to predict such a 2D path by casting an appropriate prompt, we find that standard pre-trained VLMs struggle with predicting such a path in a zero-shot manner (see \Cref{tab:experiments:vlm}). Therefore, we finetune pre-trained VLMs on datasets that ground VLMs to robot scenes and path predictions collected from easier-to-obtain sources, i.e., internet visual-question-answering data, robot data from other modalities, and simulation data.
% \footnote{Data sources such as human image annotations or end effector trackers on robot videos can also be used.} 
The primary advantages of finetuning such a hierarchical VLM that produces intermediate representations $\hat{p}_i$ compared to producing actions $a$ with a monolithic model~\citep{kim2024openvla, zitkovich2023rt} are twofold: 1) the lack of actions in certain off-domain datasets (such as videos) makes it impossible to even train monolithic pixel-to-action models, 2) we find that hierarchical VLMs producing intermediate cross-domain predictions generalize more effectively than monolithic VLAs. 

\textbf{Finetuning Objective and Datasets.}
\label{sec:method:vlm:datasets}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figs/robolines_training_data.pdf}
%     \caption{(a): Examples of training data in $\Tilde{\mathcal{D}}_\text{off}$ used to train \method's VLM. (b): The data used to train \method's low-level policies
%     % \ankit{show one example of each of the training data domain used in training the VLM (3 images like in the text); show a couple of examples of the training data used for training the policy. show the input/output for both cases.}
%     }
%     \label{fig:experiments:training_data}
% \end{figure}
% The 2D path that the VLM predicts is represented sequence of tokens corresponding to points on an image that detail where the robot gripper should move and close/open to complete the task (see \Cref{fig:method}(a)).
We use VILA-1.5-13b~\citep{vila2024}, a 13-billion-parameter vision language model trained on interleaved image-text datasets and video captioning data, as our base VLM. We then curate a multi-domain dataset to finetune this model for effective 2D path prediction. Predicting the 2D path of the end-effector requires understanding \emph{what} objects to manipulate in a given task in terms of their pixel positions, but also reasoning about \emph{how} a robot should perform the task. To enable this understanding, we collate a diverse off-domain dataset $\vlmdata$ from a wide range of modalities, including real-world data, visual question-answering data, and simulation data. Importantly, \emph{none} of this off-domain data used to train the VLM comes from the deployment environment, thereby emphasizing generalizability. However, as outlined in \Cref{sec:method:policy}, the predictions of this trained VLM are used to guide a low-level policy at inference time. 
%are paired with a small amount of in-domain trajectory data $\mathcal{D}$ to train low-level control policies. \anqi{Maybe a stupid Q since I am not fully aware of the techinical details. Did we use the VLM outputs to train the low-level policy or the GT eef 2D paths?}

We assemble a dataset $\Tilde{\mathcal{D}}_\text{off} = \{(o_i^o, z_i^o, p_i^o)\}_{i=1}^M$ of image inputs $o^o_i$, language prompts $z_i^o$, and path labels $p_i^o$ consisting of three types of data: (1) pixel point prediction tasks (\emph{what}); (2) simulated robotics tasks (\emph{what and how}); (3) a real robot dataset consisting of trajectories (\emph{what and how}). 
We detail each dataset below; see \Cref{fig:experiments:training_data} for visualization of each dataset's prompts and labels.

\textbf{Pixel Point Prediction.} For pixel point prediction, we use the dataset released by RoboPoint~\citep{yuan2024robopoint} with 1.4 million VQA tasks, with most answers represented as a list of 2D points corresponding to locations on the image. A sample consists of a prompt $z^o$ like $\texttt{Find all instances of cushions}$, an input image $o^o$ and labels $p^o$ like \texttt{$[(0.25, 0.11), (0.22, 0.19), (0.53, 0.23)]$}.
%\footnote{Note that this is not a temporally ordered path, but rather simply a set of unordered points of interest in an image. We overload notation here for the sake of notational convenience.} 
This dataset consists of data automatically generated in simulation and collected from existing real-world datasets; its diversity and tasks enable the \method\ VLM to reason about pixel-object relationships across diverse scenes while retaining its semantic generalization capabilities.

\textbf{Robot Simulation Data.} We additionally generate a dataset of simulated robotics tasks from RLBench~\citep{james2020rlbench}, a simulator of a Franka robot performing tabletop manipulation for a wide array of both prehensile and non-prehensile tasks.
We use the simulator's built-in planning algorithms to automatically generate successful manipulation trajectories and construct ground-truth 2D path labels $p^o$.
Each trajectory contains a sequence of 3D coordinates of the robot's gripper in world space, as well as whether the gripper is open or closed at a given time step. 
We use known camera intrinsics and extrinsics to project these points on the front image and construct labels $p^o = [(x_\text{image}, y_\text{image}, \texttt{gripper\_open}), \ldots]$ where $x_\text{image}, y_\text{image} \in [0, 1]$ are relative pixel locations of the end effector's position on the image.
% \anqi{should also explain what {\tt gripper\_open} is}. 
The front camera image of the initial state forms the image input $o^o$ and the prompt $z^o$ for the VLM is to provide a sequence of points denoting the trajectory of the robot gripper to achieve the given instruction (see Figure~\ref{fig:method})
We generate 1000 episodes for each of 79 robot manipulation tasks in RLBench, each episode with $\sim$4 language instructions, for a total of $\sim$300k $(o^o, z^o, p^o) $ tuples for $\Tilde{\vlmdata}$.

\textbf{Real Robot Data.} Using real robot data allows us to ensure the VLM can reason about objects and robot gripper paths when conditioned on scenes, including real robot arms.
We use existing, online robot datasets \emph{not from the deployment environment} to enable this VLM ability.
We source 10k trajectories from the Bridge dataset~\citep{walke2023bridgedata, open_x_embodiment_rt_x_2023} consisting of a WidowX arm performing manipulation tasks and \~45k trajectories from DROID~\citep{khazatsky2024droid}. 
For both datasets, we use the given end-effector trajectories and given (or estimated) camera matrices to convert robot gripper trajectories to 2D paths $p^o$. We use a camera image from the first timestep of each robot trajectory as $o^o$ and a similar text prompt $z^o$ as the simulation dataset. Note that we essentially utilize the robot data as video data, where the end effector is tracked over time. In principle, this could be done with any number of point-tracking methods~\citep{doersch2023tapir} on raw video as well, with no action or proprioceptive labels. 

\textbf{VLM Training.}
We finetune the \method\ VLM on all three datasets by randomly sampling from all samples in the entire dataset with equal weight.
%\jz{Yi fill in weighting scheme} \yi{most of the strategy is similar to sft step in VILA. we use VILA1.5-13B as pretrained weight which uses Vicuna-1 as LLM and siglip-so400m-patch14-384 as vision encoder. 
%We finetune both LLM and vision encoder. since we are using equivalent batch size 256 instead of 2048, we use LR=1e-5 instead of 1e-4 to maintain stable loss curve. It takes 30 hours on an 8xA100 node.} 
%sampling weights with the standard VLM training objective of minimizing the negative log-likelihood of the answer tokens $p_\text{ans}$ conditioned on prompt tokens $p_\text{prompt}$ and an input image $o$:
One problem with directly training on the path labels $p^o$ is that many paths may be extremely long, e.g., exceeding one hundred points. 
Since we want the \method\ VLM to reason at a \emph{high level} instead of on the same scale as the low-level control policy.
Therefore, we simplify the paths $p^o$ with the Ramer-Douglas-Peucker algorithm~\citep{RAMER1972244, douglas_pecker_1973} that reduces curves composed of line segments to similar curves composed of fewer points. 
% This results in an average 2D path length consisting of \jz{yi insert} points.
We train with the standardized supervised prediction loss to maximize the log-likelihood of the language labels $p^o$:
% \anqi{ground truth labels or 2D points/paths labels? With language, one may confuse it with $z$.}:
%\begin{equation*}    
$\mathbb{E}_{(o^o_i, z_i^o, p_i^o) \sim \Tilde{\vlmdata}}  \log \text{VLM} \left( p_i^o \mid z_i^o, o^o_i \right).$
%\end{equation*}

\subsection{Path Guided Low-Level Policy Learning}
\label{sec:method:policy}
After training the \method\ VLM to predict paths, we train a low-level policy to utilize these paths to predict actions. While a low-level control policy \emph{can} learn to solve the task without access to 2D path predictions, providing it with 2D paths can make the task easier. The paths allow the low-level policy to forgo long-horizon and semantic reasoning and focus on local and geometric predictions to produce low-level actions. As we find empirically (see \Cref{fig:experiments:main_exp}), 2D paths allow for considerably improved visual and semantic generalization of low-level policies. We train low-level policies based on rich 3-D perceptual information, available at test time on a robotic platform with standard depth cameras. Then the question becomes---how do we incorporate 2D path information $\hat{p}$ produced by the VLM in \Cref{sec:method:vlm:datasets} onto the 3D inputs to enable generalizable robot manipulation? 
% We first provide a description of low-level policy training guided by path information and then detail how the VLM and low-level policy are combined into our \method\ VLA for evaluation in the real world.

% \subsubsection{Training Path-Conditioned Policies}
% \label{sec:method:policy:training}
\textbf{Conditioning on Paths.}
We convert 2D paths of the form $p = \{(x_i, y_i, \texttt{gripper\_open})\}_{t=1}^L$ into a format that is easy to incorporate into any language ($z$), proprioception ($s$), and image ($o$) conditioned policy $\pi_\theta(a \mid s, o, z)$.
% while also ensuring the paths are represented in a natural manner that is easy to learn from? 
While one could concatenate the path with the proprioception or language input, paths are of varied lengths, and this could prevent the integration of such paths into existing policy architectures that cannot take in varied proprioceptive or language inputs. Instead, we directly draw the 2D path points onto the image input to the policy, which is not only generalizable across policy architectures but also may provide easier-to-follow path guidance as the policy does not have to learn how to associate path points with their corresponding image locations~\citep{gu2023rttrajectory}. 
During training, we use oracle paths constructed by projecting end-effector points to the camera plane as described for simulation and real robot data in \Cref{sec:method:vlm:datasets}.

Formally, we iterate 
% \anqi{need to clarify how the paths are obtained. Is it through path-labeler or VLM? Need to use $\hat{l}_i$ later on if we use VLM predictions.} 
through each trajectory $\tau_i = \{s_i^t, a_i^t, o_i^t, z_i)\}_{t=1}^T$ on the in-domain dataset $\mathcal{D}$ to obtain the path $p_i$. 
% \anqi{somehow similar confusion here} describing $\tau_i$. 
\citet{gu2023rttrajectory} proposed using colored trajectories to guide a policy's actions, and we largely follow their method of coloring trajectories to indicate gripper status and progression through time. 
These paths are drawn onto all images in the trajectory $o_i^1...o_i^T$ by drawing points at each $(x, y)$ and connecting them with line segments to obtain $\{\tilde{o}_i^t\}_{t=1}^T$.
We use a color gradient to indicate progression through time (see \Cref{fig:method}(b) for an example).
We plot circles for change in gripper status: e.g., \textcolor{green}{green} for closing the gripper and \textcolor{blue}{blue} for opening.
This constructs the final in-domain path-labeled dataset $\mathcal{D}_\text{path} = \{ (s_i, a_i,\tilde{o}_i, z_i)\}_{i=1}^N$.
% \anqi{Earlier in 4.1, $\mathcal{D}$ is used to also refer to the path-labeled dataset, and I suggested to change it to $\Tilde{\mathcal{D}}$. Either way, we need to make it consistent.}


%$ = \{ (s_i, a_i, o_i, z_i) \}_{i=1}^N$ 

%\ag{TODO: we need to describe this more formally and potentially for both 3D-DA type methods and for RVT style methods}
%\ag{We need to argue why this is better than just concatenating etc}


%Describe the shallow head architecture and how exactly the trajectory is fed into the low-level policy (image overlay). Describe how this can be trained on in-robot data. I wouldn't make it too specific to RVT or 3DDA or anything. Just as a general low-level policy. 

%\subsubsection{Training the Policy}
\textbf{Imitation Learning.} Finally, we train a policy $\pi_\theta(a \mid s, \tilde{o}, z)$ 
% \anqi{is it conditioned on $z$ or $l$? Isn't $l$ given by $\tilde{o}$ already?} 
conditioned on proprioception and other sensor information $s$, path-annotated image observations $\tilde{o}$, and a task language instruction $z$ on $\mathcal{D}_\text{path}$.
% \anqi{reminder on notation consistency for this dataset}. 
\method 's general path-conditioning framework allows for using arbitrary lower-level control policies as they do not need to condition on the same inputs as the VLM.
Therefore, we train 3D low-level policies, such as RVT-2~\citep{goyal2024rvt} and 3D-DA~\citep{ke20243d}, for low-level control.
Here, we assume $s$ includes additional sensor information (i.e., depth),
% \anqi{I think earlier in Section 3, $p$ is explicitly refered to as proprioceptive information, which by definition does not include perception input. Maybe explicitly adding depth or instead say that depth is also included in observation $o$?}
which 3D-DA and RVT-2 utilize to construct point clouds and virtual camera renderings, respectively, for more accurate control and data-efficient imitation learning.
We directly train these policies, with no necessary architectural changes,
%\footnote{We ignore the language instruction for RVT-2 it is already encoded in the 2D path.} 
with their supervised imitation learning objectives on $\mathcal{D}_\text{path}$
% \anqi{reminder on notation consistency for this dataset} 
to maximize log-likelihoods of the dataset actions: $\mathbb{E}_{(s_t, a_t, \tilde{o}_t, z_t)\sim \mathcal{D}_\text{path}} \log \pi_\theta(a \mid s_t, \tilde{o}_t, z_t)$. 
% \anqi{reminder on notation consistency for this dataset}
For further implementation details, see \Cref{sec:appendix:implementation}.



\textbf{Online Evaluation.}
% \label{sec:method:evaluation}
% Finally, we describe how we generate low-level actions with the \method-VLA architecture at inference time. 
Standard VLA architectures query the VLM for every low-level action~\citep{kim2024openvla, rt22023arxiv}, which can be very expensive with large VLMs---for example, OpenVLA's 7B param VLA only runs at 6Hz on an RTX 4090~\citep{kim2024openvla}.
Instead, \method 's hierarchical design allows us to query the VLM just once at the beginning of the episode to generate a 2D path $\hat{l}$ that we draw onto every subsequent image.
%\footnote{\method\ is not inherently limited to being queried once per episode, but for simplicity and computational efficiency we query just once per episode in our experiments.}
Therefore, \method\ can be scaled to large VLM backbones without needing end-users to be concerned about inference speed.

% % During downstream evaluation in the target environment, we query the \method\ VLM  once at the start of the episode to generate a 2D path given the first observation $o_1$. 
% These 2D paths are then drawn onto all future frames $\tilde{o}_{1:N}$ for $\pi_\theta$ as described in \Cref{sec:method:policy:training}. See \Cref{fig:method} for a visualization of the full online evaluation pipeline.

% To summarize, we finetune a VLM on cross-modal, cheaply obtained data from the internet to predict trajectory keypoints \anqi{2d paths} to annotate images for an image-conditioned policy to receive high-level trajectory guidance to perform low-level control. \anqi{Avoid one-sentence paragraphs.}


==> sections/related_work.tex <==


\section{Related Work}

\paragraph{Brainstorming below.}
Maybe: Training VLMs to output trajectory-level representations can help make simulation data useful for the real world.
\begin{itemize}
    \item \textbf{RoboPoint}~\citep{yuan2024robopoint}: This work focuses on training a VLM for predicting relevant points on an image. These points could potentially be used for downstream applications like Manipulation. In contrast, we predict end-effector trajectory using a VLM and then use it to aid a downstream manipulation trajectory. Points could be sufficient in some applications like reaching a certain location but are insufficient for describing manipulation scenarios that require a specific movement of the end-effector like wiping a cloth.
    % Trains on sim and real data, draws points on the image for M2T2. Can train on general VQA data, but points are likely not as helpful as full trajectories as an interface between VLMs and policies in general (we should show this). \yi{I think it is OK since we can just say point is another format of cheap data}
    
    \item \textbf{LLARVA}~\citep{niu2024llarva}: LLARVA also explores the use of trajectories. They 2D-trajectory prediction task could serve as an additional source of supervision. However, they predict action via an end-to-end Vision Action Model. We on the other hand study an explicit hierarchical design, where 2D-trajectory from a VLM is fed to an action model for predicting actions. 
    % Pre-trained on Open-X~\citep{o2024open}, then fine-tuned for the specific downstream task. Needs a crazy amount of downstream fine-tuning data. Predicts 2D traces as an auxiliary loss for using the VLM as a VLA with robot actions. Ablations show it helps.
    \item \textbf{RT-Trajectory}~\citep{gu2023rttrajectory}: RT-Trajectory is a closely related work which proposes to use a trajectory for communication. However, there are a couple of differences:
    -- they do not explore or develop a VLM for trajectory generation; use off the shelf which is worse; 
    -- they only consume the trajectory with a large action model like RT. In our design any action head can be used including relatively small 3D action head. Our proposal is to use the design as being more general than being specific to RT. \caelan{Are there specific aspects of training our own VLM that make it more adept in the hierarchy (other than just training on the trajectory dataset)}
    % \emph{proposes} sketches for policy conditioning. Trains with hindsight-labels but does inference exps with human drawings, human hand capture, and LLMs/VLMs. VLM: image $\rightarrow$ 2d image pos tokens, without fine-tuning. Just evaluates on 1 RT-1 style policy arch.
    % \item \textbf{MotIF: Motion Instruction Fine-tuning}~\citep{hwang2024motifmotioninstructionfinetuning}: Fine-tunes VLMs for detecting success on drawn trajectory motions of robots rather than single image states. Not too too related. [too recent, no need to compare]
    \item \textbf{KITE: Keypoint-Conditioned Policies for Semantic Manipulation}: Yes, they also have a two stage design like us. But only marks points instead of trajectory; explore the use of a prefixed library of action primitives instead of a learned policy model.
    \item \textbf{Robot-Moo: Open-World Object Manipulation using Pre-Trained Vision-Language Models} Similar to KITE -- marks only object bounding boxes.
    \item \textbf{Flow as the Cross-Domain Manipulation Interface} Generates object-centric flow; We instead create robot-centric trajectory; [To Check: Does not consider open-world generalization?]
    \item \textbf{Any-point trajectory modeling for policy learning} \yi{this and the above one, these two are prediction short term flow, which still needs full trajectory and not easy to scale up}
    \item \textbf{MOKA: Open-World Robotic Manipulation through Mark-Based Visual Prompting} Another way of prompting VLMs, complementary to our idea and can be used within our design, we compare training a VLM vs prompting.
    \item \textbf{PIVOT: Iterative Visual Prompting Elicits Actionable Knowledge for VLMs} Another way of prompting VLMs, complementary to our idea and can be used within our design, we compare training a VLM vs prompting.
    \item \textbf{RAM: Retrieval-Based Affordance Transfer for Generalizable Zero-Shot Robotic Manipulation} different type of method - retrieval vs learning
    \item \textbf{OPTIMUS~\citep{dalal2023imitating}}: train BC agents on cheap data procedurally generated in simulation (using a task and motion planning system)
    \item \textbf{HITL-TAMP~\citep{garrett2021integrated,mandlekar2023human}}: hierarchical policy that uses Task and Motion Planning (TAMP) at the high level and BC agents at the low level
    % Also, MimicGen, SkillGen, etc.
\end{itemize}

Other:
\begin{itemize}
    \item Peract/RVT~\citep{shridhar2023perceiver,goyal2023rvt,goyal2024rvt} ...
    \item 3DDA~\citep{gervet2023act3d,ke20243d} ...
    \item GPT-4V~\citep{openai2024gpt4} ...
    \item SayCan~\citep{brohan2023can} ...
    \item ProgPrompt~\citep{singh2023progprompt} ...
\end{itemize}


==> sections/related_work_workshop.tex <==
\section{Related Work}
\textbf{LLMs and VLMs for robotics.} 
Early attempts in leveraging LLMs and VLMs for robotics are through pretrained language~\citep{jang2022bc,shridhar2023perceiver,singh2023progprompt} and visual~\citep{shah2021rrl,parisi2022unsurprising,nair2023r3m,ma2023vip} models. However, these are not sufficient for complex semantic reasoning and generalization to the open world~\citep{brohan2022rt,zitkovich2023rt}. Recent research has focused on directly leveraging open world reasoning and generalization capability of LLMs and VLMs, by 
prompting or fine-tuning them to, e.g., generate plans~\citep{huang2022language,huang2023inner,lin2023text2motion,liang2023code,singh2023progprompt,brohan2023can}, construct value~\citep{huang2023voxposer} and reward functions~\citep{kwon2023reward,RoboCLIP,yu2023language,ma2024eureka,wang2024rl}. Our work is more closely related to the literature on VLA models, summarized below.

\textbf{Monolithic VLA models as language-conditioned robot policies.}
Monolithic VLA models have been proposed to produce robot actions given task description and image observations directly \citep{brohan2022rt,jiang2023vima,zitkovich2023rt,team2024octo,kim2024openvla,radosavovic2023robot}. Monolithic VLA models are often constructed from VLMs~\citep{liu2024visual,bai2023qwen,driess2023palm,vila2024}, and are trained on large-scale robot teleoperation data~\citep{brohan2022rt,open_x_embodiment_rt_x_2023,khazatsky2024droid} to predict actions as text or special tokens. However, due to the lack of coverage in existing robotics datasets, they must be finetuned in-domain on expensive teleoperated data. The most relevant monolithic VLA model is LLARVA~\citep{niu2024llarva}, which predicts end-effector trajectories in addition to robot actions. However, LLARVA does not use trajectory prediction to control the robot; rather, it uses it as an auxiliary task to improve action prediction. Therefore, LLARVA still suffers from the limitations of monolithic VLA models. In contrast, our work takes a hierarchical approach, drastically reducing the number of demonstrations needed for learning downstream tasks and the number of VLM calls per episode. Moreover, our proposed hierarchical architecture enables training from cheaper data sources while enabling considerable cross-domain transfer. 

\textbf{VLMs for predicting intermediate representations.}
Our work bears connections to prior methods using vision-language models for intermediate prediction. These methods can be categorized by the choice of predicted representation:

% \anqi{I actually feel that we should uncomment the previous sentence to so that we don't have a one-sentence paragraph.}

\emph{Point-based predictions:} A common intermediate prediction interface has been keypoint affordances~\citep{stone2023open,sundaresan2023kite,nasiriany2024pivot,yuan2024robopoint}. Some examples include using open-vocabulary detectors~\citep{minderer2022simple}, iterative prompting of VLMs~\citep{nasiriany2024pivot}, or fine-tuning detectors to identify certain parts of an object by semantics~\citep{sundaresan2023kite}. Perhaps most related, \cite{yuan2024robopoint} finetunes a VLM to predict objects of interest as well as free space for placing an object, and \cite{liu2024moka} propose a mark-based visual prompting procedure to predict keypoint affordances as well as a fixed number of waypoints. As opposed to these, our work finetunes a VLM model to not just predict points but rather entire 2D paths, making it more broadly applicable across robotic tasks. 

\emph{Trajectory-based predictions:} The idea of using trajectory-based task specifications to condition low-level policies was proposed in RT-trajectory~\citep{gu2023rttrajectory}, largely from the perspective of flexible task specification. This work also briefly discusses the possibility of combining RT-Trajectory with trajectory sketches generated from prompting a pre-trained vision language model. Complementary to RT-Trajectory, the focus of this work is less on the use of trajectory sketches for task specification, but rather on the abilities of a hierarchical VLA model to finetune the high-level VLM on cheap and abundant sources. %This could include training data such as videos or simulation data, and show transfer to test scenarios of interest with considerable visual and semantic variation. 
While RT-trajectory uses human effort or off-the-shelf pre-trained models to generate trajectories, we show that finetuning VLM models on cheap data sources can generate more accurate and generalizable trajectories (see Table.~\ref{tab:experiments:vlm}). Moreover, our instantiation of this architecture enables the incorporation of rich 3D and proprioceptive information, as compared to monocular 2D policies~\citep{gu2023rttrajectory}. 

==> tables/ablation.tex <==
\begin{table}[t]
\centering % Ensures the table is centered in the wraptable environment
\caption{Comparison on critical point accuracy between HAMSTER (ours) and HAMSTER where the VLM is trained to predict dense path points.}
\label{tab:dense_traj_comparison}
% \resizebox{\linewidth}{!}{% Adjust the width as needed
\begin{tabular}{l|c}
\hline
\textbf{Method}                & \textbf{Acc (\%)} \\
\hline
\method + Dense Path & xx.xx  \\ 
\method                      & xx.xx  \\
\hline
\end{tabular}
% }
\end{table}


==> tables/rebuttal_sim_table.tex <==
% %\begin{table}[h!]
% \begin{wraptable}[8]{R}{0.35\textwidth}
% \centering
% \vspace{-0.5cm}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lc}
% \toprule
% \textbf{Method} & Success \\ \midrule
% 3D-DA & 0.18 $\pm$ 0.10                     \\ 
% \method+3D-DA (50\%) & 0.36 $\pm$ 0.04                    \\ 
% %\method+3D-DA (Open/Close) & 0.39 $\pm$ 0.05                    \\ 
% \method+3D-DA & \textbf{0.43 $\pm$ 0.05}                    \\ \bottomrule
% \end{tabular}
% }
% %\vspace{-0.3cm}
% \caption{\footnotesize{Colosseum results demonstrate that \method\ is demo-efficient, doubling 3D-DA's success rate even with just 50\% of the data.}}
% \label{tab:rebuttal_sim_table}
% %\end{table}
% \end{wraptable}

==> tables/view_invariance.tex <==
% \begin{table}[t]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method}         & \multicolumn{2}{c}{\textbf{Original Camera}} & \multicolumn{2}{c}{\textbf{Novel Camera}} \\
% \cmidrule{2-3} \cmidrule{4-5} 
%                         & Success Score & Full Success & Success Score     & Full Success \\ \midrule
% OpenVLA                & 6                  & 3                        & 2.25               & 0                        \\ 
% HAMSTER+RVT2           & 8.25               & 7                        & 7.25               & 4                        \\ 
% HAMSTER+RVT2 (Concat)  & \textbf{10}        & \textbf{10}              & \textbf{9.75}      & \textbf{9}              \\ \bottomrule
% \end{tabular}
% %\vspace{-0.4cm}
% \caption{\footnotesize{Real world results comparing \method, \method\ where paths are concatenated with RGB instead of drawn onto the image, and OpenVLA on a setup with the new camera angle as shown in \Cref{fig:camera_angle}. We report cumulative completion scores out of 10 (10 trials) and total number of fully successful executions. \method\ performs better with both path drawing settings.}}
% \label{tab:camera_comparison}
% \end{table}

==> tables/vlm_workshop.tex <==
\begin{table}[!tb]
\centering
\resizebox{0.8\linewidth}{!}{% Adjust the width as needed
    \begin{tabular}{llllll}
    \toprule
    Method & VLM & Finetuning  Data & Rank Exc. Real RLB. & Rank Real RLB. & Rank All \\
    \midrule
    RT-Traj.  & 0-shot GPT-4o & - & 3.40 & 3.63 & 3.52 \\
    RT-Traj.  & CaP GPT-4o & - & 3.57 & 3.36 & 3.46 \\
    \method \ & VILA & Our Exc. Sim RLB. & 1.78 & 2.39 & 2.11\\
    \method \ & VILA & Our & \textbf{1.59} & \textbf{1.28} & \textbf{1.42}\\
    
    \bottomrule
    \end{tabular}
}
\caption{\footnotesize{Ranking-based human evaluation of different VLMs, averaged across various real-world evaluation tasks. Results indicate that \method\ including simulation data is most effective since it captures both spatial and semantic information across diverse tasks from RLBench (RLB). 
%This significantly outperforms zero-shot VLM-based trajectory generation, as described in \citet{gu2023rttrajectory}}}
}}
\label{tab:experiments:vlm}
\end{table}

